CITADEL: Conditional Token Interaction via Dynamic Lexical Routing for Efficient and Effective Multi-Vector Retrieval

Multi-vector retrieval methods combine the merits of sparse (e.g. BM25) and dense (e.g. DPR) retrievers and have achieved state-of-the-art performance on various retrieval tasks. These methods, however, are orders of magnitude slower and need much more space to store their indices compared to their single-vector counterparts. In this paper, we unify different multi-vector retrieval models from a token routing viewpoint and propose conditional token interaction via dynamic lexical routing, namely CITADEL, for efficient and effective multi-vector retrieval. CITADEL learns to route different token vectors to the predicted lexical ``keys'' such that a query token vector only interacts with document token vectors routed to the same key. This design significantly reduces the computation cost while maintaining high accuracy. Notably, CITADEL achieves the same or slightly better performance than the previous state of the art, ColBERT-v2, on both in-domain (MS MARCO) and out-of-domain (BEIR) evaluations, while being nearly 40 times faster. Code and data are available at https://github.com/facebookresearch/dpr-scale.

==> Makefile <==
engine = "pdflatex -interaction=nonstopmode --shell-escape %O %S"
refs = references.bib
# sources = main.tex $(wildcard **/*.tex)
# sources = main.tex $(shell find -print **/*.tex)
sources = main.tex $(shell find . -type f -name '*.tex')

main.pdf: $(sources)
	@latexmk -pdf -pdflatex=${engine} -output-directory='output' -bibtex $<

watch:
	make; \
	(zathura output/main.pdf &); \
	while true; do \
		inotifywait -e modify -q $(sources); \
		make; \
	done
	# @while inotifywait -e modify $(refs) $(sources); do make; done

spell:
	@hunspell -l -t -d en_US -i utf-8 $(sources) \
		| sort \
		| uniq --ignore-case \
		| grep -vxFf dictionary.txt

clean:
	@latexmk -C
	rm -rf output/*

pack:
	rm ../active-inference.tar || true
	cp output/references.bbl references.bbl
	tar -czvf ../active-inference.tar --exclude .git --exclude .gitignore --exclude *.log --exclude output .

.PHONY: watch spell clean


==> sections/acknowlegement.tex <==
\section{Acknowledgement}
Jun Yan, Zheng Lian

==> tables/openqa.tex <==
\begin{table*}[!t]
\centering
% \hspace*{-1cm}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|cc|cc|c|cc|ccc}
\toprule
\textbf{Models}& \multicolumn{2}{c|}{\textbf{NQ}}& \multicolumn{2}{c|}{\textbf{TQA}} &\multicolumn{1}{c|}{\textbf{Entity}} & \multicolumn{2}{c|}{\textbf{Index Storage}}& \multicolumn{3}{c}{\textbf{Latency (ms/query)}}\\
& \small{Rerank} &\small{Retrieval} & \small{Rerank} &\small{Retrieval} &\small{Retrieval} &\small{Disk (GB)} &\small{Factor} &\small{Encode (GPU)} &\small{Search (GPU)} &\small{Search (CPU)}\\
\midrule
BM25 (Anserini) &0.629 &0.629 &0.764 &0.764 \\
DPR-768 &0.794 &- &0.785 &- \\
DPR-128 &0.720 &- &0.699 &- \\
SPLADE & 0.801 &- &0.820 &-\\
COIL-tok &0.790 &- &0.818 &-\\
COIL-full &0.798 &- &0.825 &- \\
ColBERT-$\text{QA}_1$ &\textbf{0.810} &- &\textbf{0.830} &- \\
CITADEL &0.781 &- &0.817 &-\\
CITADEL (w/o reg.) &0.796 &- &\textbf{0.830} &-  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{In-domain evaluation on Natural Questions and TriviaQA, as well as out-of-domain evaluation on Entity QA. Top-20 Accuracy are reported. Reranking is performed on top-1000 retrieval results of BM25.}
\label{tbl:openqa}
\end{table*}
